Shem: A Hardware-Aware Optimization Framework for Analog Computing Systems

As the demand for efficient data processing escalates, reconfigurable analog hardware which implements novel analog compute paradigms, is promising for energy-efficient computing at the sensing and actuation boundaries. These analog computing platforms embed information in physical properties and then use the physics of materials, devices, and circuits to perform computation. These hardware platforms are more sensitive to nonidealities, such as noise and fabrication variations, than their digital counterparts and accrue high resource costs when programmable elements are introduced. Identifying resource-efficient analog system designs that mitigate these nonidealities is done manually today. While design optimization frameworks have been enormously successful in other fields, such as photonics, they typically either target linear dynamical systems that have closed-form solutions or target a specific differential equation system and then derive the solution through hand analysis. In both cases, time-domain simulation is no longer needed to predict hardware behavior. In contrast, described analog hardware platforms have nonlinear time-evolving dynamics that vary substantially from design to design, lack closed-form solutions, and require the optimizer to consider time explicitly. We present Shem, an optimization framework for analog systems. Shem leverages differentiation methods recently popularized to train neural ODEs to enable the optimization of analog systems that exhibit nonlinear dynamics, noise and mismatch, and discrete behavior. We evaluate Shem on oscillator-based pattern recognizer, CNN edge detector, and transmission-line security primitive design case studies and demonstrate it can improve designs. To our knowledge, the latter two design problems have not been optimized with automated methods before.

==> sections/compiler.tex <==
\section{The \tool{} Compiler}

\subsection{Compile dynamical graph to ODEs}

\iffalse
\subsection{Algebraic rewrite}
There are two main reasons for rewriting an analog computation, for convergence of the optimization and for numerical precision.
Previous studies in neural network training have shown that normalization is critical for the convergence of stochastic gradient descent~\cite{ioffe2015batch, salimans2016weight}. From this intuition, we would like the free variables in the analog circuits to have the same scale. Additionally, (maybe) empirical results suggest that having variables in the denominators will slow the convergence. Therefore, we want to ``normalize" the variables such that they are at the denominators in the computation.

Solving ordinary differential equations accurately is critical for circuit simulation, which can usually be achieved with high-precision floating point, e.g. 64-bit. Ideally, one can also use high-precision floating-point representation when optimizing differential equation parameters with gradient descent. However, practical accelerators (e.g., GPU, TPU) for gradient descent-based optimization are moving toward low-bitwidth representation~\cite{XXX}. We observed an accuracy issue in the ODE-solving when naively using low-precision floating points. Therefore, two rewritings are deployed to improve the numerical stability: rescaling the state variables and replacing operators with numerical-friendly implementations.

In sum, we would like the analog circuit computation to have the following properties.
\begin{itemize}
    \item \textbf{Unit weights.} All the free variables are within range [-1, 1]
    \item \textbf{Weights in the denominator.} All the free variables are at the denominator of the computation
    \item \textbf{``Small" state variables and derivatives.} Values in the computation should be scaled to close to the origin instead of being large values.
\end{itemize}


\subsubsection{Unit normalization and symbolic simplification}
Rescale all trainable parameters to unit scale. Replace every denominator with its inverse (safe because parameter bounds are required).

For example,
\begin{equation}
    \begin{cases}
        \ddt{x} = \frac{a\cdot x}{C} + \frac{b\cdot y}{C} \\
        \ddt{y} = \frac{d\cdot x}{L} + \frac{e\cdot y}{L}
    \end{cases}
\end{equation}
After symbolic simplification, the system becomes
\begin{equation}
    \begin{cases}
        \ddt{x} = C'(a\cdot x+ b\cdot y) \\
        \ddt{y} = L'(c\cdot x+ d\cdot y)
    \end{cases}
\end{equation}
Say $C, L \in [10^{-10}, 10^{-8}]$ and $a,b,c,d\in[0, 4]$. The unit normalization yields
\begin{equation}
    \begin{cases}
        \ddt{x} = 10^{C''-9}(2(a'+1)\cdot x+ 2(b'+1)\cdot y) \\
        \ddt{y} = 10^{L''-9}(2(c'+1)\cdot x+ 2(d'+1)\cdot y)
    \end{cases}
\end{equation}
so that $C'', L'',a',b',c',d'\in[-1, 1]$ (note that the normalization form is different between $LC$ and $abcd$). Can we rescale the whole dynamical system so that all terms are on the same scale? Won't know the range of state variables ($xy$) easily if arbitrary nonlinearity is involved.

What if the denominator is not separable?
\begin{equation}
    \begin{cases}
        \ddt{x} = \frac{a\cdot x}{C + by} \\
        \ddt{y} = \frac{d\cdot x}{L + ey}
    \end{cases}
\end{equation}

Rescale time and state variables. For general ordinary differential equations, $\ddt{x}=f(x,t), x(0)=x_0, t\in[0,t_M]$. Say $\Bar{x}=\frac{x}{x_c},\Bar{t}=\frac{t}{t_c}$. We have
\begin{equation}
    \frac{d\Bar{x}}{d\Bar{t}}=\frac{d\Bar{x}}{dx}\ddt{x}\frac{dt}{d\Bar{t}}=\frac{1}{x_c}f(x_c\Bar{x},t_c\Bar{t})t_c, \Bar{x}(0)=\frac{x_0}{x_c}
\end{equation}
In general, we can support two invertible scaling matrices.
If $t_c$ and $x_c$ appear at the outmost of the equations, can choose them to cancel the unit normalization terms.


\subsubsection{Lump parameters}
\fi

\subsection{Compile smooth approximation}

\subsubsection{Device-to-value lookup table}
Use interpolation
\subsubsection{Discrete parameters}
For simulation, it is the same as continuous parameters. Need special care for optimization, e.g., interpolation as a LUT or tricks like Gumbel-Softmax.
\subsubsection{Noise injection}
Add \codein{noise} symbol in production rules that represents a white noise with unit standard deviation. Can have arbitrary expression before \codein{noise} to denote the amplitude. The compiler will collect the noise terms within a node and express the total noise amplitude as the root-mean-squared sum of amplitudes.

\iffalse
\subsection{Library-specific compilation}
\subsubsection{Rewrite with library api}
Operation in the numerical computing library is more efficient and accurate. For example, reduction of summation or multiplication is replaced with "jnp.sum" and "jnp.multiply"
\fi


\subsection{}

==> sections/introduction-scratch.tex <==




Analog computing paradigms show promise in enabling 1. highly resource-efficient computation and optimization, and 2. in/near- sensor computation, serving as an effective preprocessing mechanism for classical image and sound machine learning tasks to minimize data transfer...

However, a comprehensive co-design framework is absent. Previous efforts in hardware-algorithm co-design have been tailored to specific hardware units, thereby 1. posing challenges for non-hardware domain specialists, such as machine learning experts, to engage effectively in the co-design process, and 2. requiring laborious manual analysis of hardware to set up the co-design. Moreover, the methodologies developed in each project are not readily adaptable to other hardware-algorithm co-design challenges due to their specificity to the targeted hardware...

We introduced \tool{}, a framework to enhance collaboration between analog hardware designers and domain specialists, focusing on differentiable circuit modeling and optimization. \tool{} builds upon Ark~\cite{XXX}, which offers a graph-based intermediate representation accessible to both parties, enabling the encoding of analog computing paradigms and the analog circuit design space into domain-specific languages (DSLs). Building upon Ark, \tool{} endows the following capabilities.



\subsection{System overview}

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/ArkOpt-Overview.pdf}
    \caption{Overview of analog computing paradigm optimization with \tool{}.}
    \label{fig:enter-label}
\end{figure}


Optimize physical system vs. neural network
contribution: the processes to make the 


\todo{Practical consideration: Justify no hardware validation yet. Point out previous work Ark allow freely specifying models and this work demonstrate optimizing in the high-level... Do not target any specific technology or devices. Future work is working with analog designer? How to phrase this?}

\subsection{Analogy Between Analog Compute Paradigms and Neural Networks: \obc{} Example}
The key insight of this work is the analogy between neural networks (\nn) and novel analog compute paradigms, enabling systematic optimization of analog computing applications under nonidealities:

\begin{itemize}
    \item \bulletkeyword{Differentiability.} Neural network (\nn) outputs are differentiable with respect to model weights. Similarly, the dynamics of the analog compute paradgims often consist of differentiable components.
    \item \bulletkeyword{Quantization.} Quantization is commonly used in neural networks to reduce computational time and energy consumption. Discrete parameters is common in analog hardware due to digital interface or switches.
    \item \bulletkeyword{Approximate Computing.} Applications in both \nn{} (e.g., image classification) and novel analog compute paradigms (e.g., pattern recognition) are error-tolerant. This means that computations need not be exact and small errors or noise are acceptable, which is distinct from conventional computing.
    \item \bulletkeyword{Emergent Behavior.} In neural networks, simple components like matrix multiplication and nonlinear activation functions combine to produce complex behaviors that are not easily inferred from the individual components. Similarly, analog systems use simple functions as building blocks, yet exhibit complex behaviors that are challenging to predict.
\end{itemize}
% Despite the similarities, a key difference between novel analog computing paradigms and \nn{} lies in execution constraints: analog computing must faithfully adhere to the underlying dynamical system model and cannot be arbitrarily modified. For instance, only the coupling weights can be (and should be) quantized, while other computations are performed in high-precision floating-point to maintain fidelity to hardware execution, where values are inherently continuous.


\subsection{Contributions}
